Can Transformers Reason Logically? A Study in SAT Solving

We formally study the logical reasoning capabilities of decoder-only Transformers in the context of the boolean satisfiability (SAT) problem. First, we prove by construction that decoder-only Transformers can decide 3-SAT, in a non-uniform model of computation, using backtracking and deduction via Chain-of-Thought (CoT). %We prove its correctness by showing trace equivalence to the well-known DPLL SAT-solving algorithm. Second, we implement our construction as a PyTorch model with a tool (PARAT) that we designed to empirically demonstrate its correctness and investigate its properties. Third, rather than \textit{programming} a transformer to reason, we evaluate empirically whether it can be \textit{trained} to do so by learning directly from algorithmic traces (``reasoning paths'') from our theoretical construction. The trained models demonstrate strong out-of-distribution generalization on problem sizes seen during training but has limited length generalization, which is consistent with the implications of our theoretical result

==> contents/acknowledgements.tex <==

\section{Acknowledgements}
This work is supported by NSF awards IIS-2229876 and CCF-2403391. The authors thank Hassan Naveed for his exploratory work on using RASP for SAT-solver implementation, William Armstrong for suggesting the abstract DPLL paper and contributing code, and Jintong Jiang for providing suggestions on the paper’s presentation and writing.

==> contents/removed.tex <==
% Define encoding $E(C) \in \{0, 1\}^{2p}$ of clause $C$ as the following: For $v\in [p]$, $E(C)_v=1$ iff $x_v$ is a literal in $C$, and $E(C)_{p+v}=1$ iff $\lnot x_v$ is a literal in $C$. All positions in $E(C)$ are $0$ otherwise.
% \end{definition}

% \begin{definition}[Encoding of partial assignment]
% \label{def:assignment_encode}
% Let $C$ be a clause in $$
% Further, $E$ maps any partial assignment $A \in \mathcal{B}$ as
% \begin{align*}
%     E(A)_v := \boldsymbol{1}_{A(x_v) = \text{True}} 
%         &\qquad\text{and}\qquad  E(A)_{v+p} := \boldsymbol{1}_{A(x_{v}) = \text{False}}; \\
%     E_{\textnormal{not-false}}(A)_v := \boldsymbol{1}_{A(x_v) \in \{\text{True}, \text{None}\}} 
%         &\qquad\text{and}\qquad  E_{\textnormal{not-false}}(A)_{v+p} := \boldsymbol{1}_{A(x_{v})  \in \{\text{False}, \text{None}\}} 
% \end{align*}  
    % $E(A) \in \{0, 1\}^{2p}$ of clause $C$ as the following: For $v\in [p]$, $E(A)_v=1$ iff $A(x_v)=\operatorname{True}$ , and $E(A)_{p+v}=1$ iff $A(x_v)=\operatorname{False}$. All positions in $E(C)$ are $0$ otherwise.


% \TODO{The above is still confusing. There needs to be some way to differentiate between $\lnot (x\in B)$ and $(\lnot x)\in B$}
% We also define a variant of the partial assignment encoding as an affine transformation of $E(A)$: $E(A)_{v} = 1$  if and only if $A(v) = \text{None}$; that is $v$ is unassigned by $A$.

% \begin{proposition}
% For partial assignment $A$, define $E_{\text{not-false}}(A) = M_{\text{not-false}} \cdot E(A) + \boldsymbol{1}^{2p}$ where $M_{\text{not-false}} = 
% \begin{bmatrix}
% \boldsymbol{0} & -\mathbf{I}_{p} \\
% -\mathbf{I}_{p} & \boldsymbol{0}
% \end{bmatrix} 
% \in \mathbb{R}^{2p \times 2p}$ and $\boldsymbol{1}^{2p}$ is the all ones vector. Then, for $v \in [p]$:
% \[
% E_{\text{not-false}}(A)_v = 1 \text{ iff } A(x_v) \in \{\operatorname{True}, \operatorname{None}\}, \quad
% E_{\text{not-false}}(A)_{p+v} = 1 \text{ iff } A(x_v) \in \{\operatorname{False}, \operatorname{None}\}.
% \]
% \end{proposition}

%To make notation easy, define the following expressions:
% \begin{align*}
%     A \models F & \text{ means the partial assignment $A$ satisfies $F$} \\
%     F\models \lnot A  & \text{ means the partial assignment $A$ contradicts $F$} \\ 
%     F\models \lnot A  & \text{ means the partial assignment $A$ contradicts $F$} \\
% \end{align*}

%The expressions we need to consider are \textit{partial assignments}, defined as a map $A: \{x_1, \dots, x_p\} \rightarrow \{\operatorname{True}, \operatorname{False}, \operatorname{None}\}$, and \textit{clauses}, defined as a subset $C$ of literals $\{x_1, \neg x_1, x_2, \neg x_2, \ldots, x_p, \neg x_p\}$; we assume without loss of generality that $C$ does not contain $x_i$ and $\neg x_i$ simultaneously for any $i$.  Let $\mathcal{B}$ be the union of the set of all partial assignments $A$ and clauses $C$. We now define how we encode objects in $\mathcal{B}$ in $\mathbb{R}^{2p}$.


% To process clauses and partial assignments with attention operations, the initial layers of the theoretical construction compute the binary vector encodings of clauses and partial assignments and store them in the hidden states. We formally define the encoding scheme for clauses and partial assignments below:

